Weakly Supervised Prototype Topic Model with Discriminative Seed Words: Modifying the Category Prior by Self-exploring Supervised Signals

Dataless text classification, i.e., a new paradigm of weakly supervised learning, refers to the task of learning with unlabeled documents and a few predefined representative words of categories, known as seed words. The recent generative dataless methods construct document-specific category priors by using seed word occurrences only, however, such category priors often contain very limited and even noisy supervised signals. To remedy this problem, in this paper we propose a novel formulation of category prior. First, for each document, we consider its label membership degree by not only counting seed word occurrences, but also using a novel prototype scheme, which captures pseudo-nearest neighboring categories. Second, for each label, we consider its frequency prior knowledge of the corpus, which is also a discriminative knowledge for classification. By incorporating the proposed category prior into the previous generative dataless method, we suggest a novel generative dataless method, namely Weakly Supervised Prototype Topic Model (WSPTM). The experimental results on real-world datasets demonstrate that WSPTM outperforms the existing baseline methods.

==> CoverLetter.tex <==
Dear Editors:

We would like to submit the enclosed manuscript entitled “Weakly Supervised Prototype Topic Model with Discriminative Seed Words: Modifying the Category Prior by Self-exploring Supervised Signals”, which we wish to be considered for publication in Information Sciences Journal. No conflict of interest exists in the submission of this manuscript, and the manuscript is approved by all authors for publication. I would like to declare on behalf of my co-authors that the work described was original research that has not been published previously, and not under consideration for publication elsewhere, in whole or in part. All the authors listed have approved the manuscript that is enclosed.

In this work, we develop a novel WSPTM method for dataless text classification with seed words. The main idea of WSPTM is to formulate a document-specific category prior, which can enrich and modify the supervision signals by self-exploring the available data and seed words. First, a novel prototype scheme is presented to better capture the label membership degree prior of documents, and second, the label frequency prior is estimated by seed word occurrences to further enrich the supervision. I hope this paper is suitable for Information Sciences Journal.

The following is a list of possible reviewers for your consideration:
1) Chuanming Song      E-mail: chmsong@163.com
2) Filipe Rodrigues    E-mail: rodr@dtu.dk
3) Saeedeh Momtazi     E-mail: momtazi@aut.ac.ir

We deeply appreciate your consideration of our manuscript, and we look forward to receiving comments from the reviewers. If you have any queries, please don’t hesitate to contact me at the address below.

Thank you and best regards.
Yours sincerely,
Ximing Li, Yue Wang, and Jihong Ouyang

Corresponding author:
Name: Ximing Li
E-mail: liximing86@gmail.com



==> Sec_Figures.tex <==
\begin{figure*}[t]
\includegraphics[width=0.9\textwidth]{Fig1.jpg}
\centering
\caption{Comparisons of the average ranks of totally $40$ evaluation results using the Nemenyi test on each evaluation metric: (a) \textbf{Micro-F1}, (b) \textbf{Macro-F1}. The comparing methods that are not significantly different at 0.05 level (i.e., \emph{p} = 0.05) are connected.}
\label{Fig1}
\end{figure*}

\begin{figure*}[t]
\includegraphics[width=0.95\textwidth]{Fig2.jpg}
\centering
\caption{The Macro-F1 scores of different $\rho$ and $\tau$ values on (a) \emph{Reuters} with $S^L$, (b) \emph{Reuters} with $S^D$, (c) \emph{Newsgroup} with $S^L$ and (d) \emph{Newsgroup} with $S^D$}
\label{Fig2}
\end{figure*}

\begin{figure}[t]
\includegraphics[width=0.45\textwidth]{Fig3.jpg}
\centering
\caption{The Macro-F1 scores of different \emph{P} values on \emph{Newsgroup} with $S^L$}
\label{Fig3}
\end{figure}



==> Sec_Tables.tex <==
\begin{table}[t]
\renewcommand\arraystretch{1.25}
\caption{A summary of notations}
\label{Notations}
\begin{center}
\begin{small}
\begin{tabular}{p{0.12\columnwidth}<{\centering}||p{0.77\columnwidth}}
\Xhline{1.2pt}
Notation & Description\\
\Xhline{1.2pt}
\hline
\hline
\Xhline{1.2pt}
\emph{D}    &   number of documents \\
\emph{K}    &   number of category topics, i.e., category labels \\
\emph{G}    &   number of background topics \\
\Xhline{1.2pt}
$\phi$      &   category topic distribution over words\\
$\widehat \phi$      &   background topic distribution over words\\
$\theta$    &   document-specific distribution over category topics\\
$\widehat \theta$    &   document-specific distribution over background topics\\
$\delta$      &  Bernoulli distribution for choosing topic type \\
\Xhline{1.2pt}
$\beta$     &   Dirichlet prior of $\phi$ \\
$\widehat \beta$     &   Dirichlet prior of $\widehat \phi$ \\
$\alpha$    &   supervised Dirichlet prior of $\theta$ \\
$\widehat \alpha$   &   Dirichlet prior of $\widehat \theta$ \\
\Xhline{1.2pt}
$\alpha'$    &   supervised Dirichlet prior of $\theta$ in \textbf{WSPTM} \\
$\rho$      &  tuning parameter of $\alpha'$\\
$\eta$      &  concentration parameter of $\alpha'$\\
$\alpha_0$  &  smoothing parameter of $\alpha'$ \\
\emph{P}    &  number of pseudo-nearest neighboring categories in the \textbf{prototype scheme}\\
$\tau$      &  tuning parameter in the formulation of document-specific label membership degree prior\\
\Xhline{1.2pt}
\end{tabular}
\end{small}
\end{center}
\end{table}


\begin{table}
\renewcommand\arraystretch{1.6}
\caption{Examples of statistics of marked labels on \emph{Reuters} (top section) and \emph{Newsgroup} (bottom section). $S^L$ and $S^D$ are two different seed word sets used in this work. $P=0$ actually implies that the prototype scheme is not applied. NonSW: the number of documents that contain no seed words, as well as marked labels. TrueMark: the number of documents, whose relevant labels belong to marked labels. TotalNum: the total number of documents.}
\label{Example}
\centering
\small
\begin{tabular}{p{40pt}!{\vrule width0.5pt}|p{45pt}p{45pt}!{\vrule width0.5pt}p{45pt}p{45pt}}
\Xhline{1.2pt}
\multirow{2}{2cm}{NumOfDoc}   & \multicolumn{2}{c!{\vrule width0.5pt}}{$S^L$} & \multicolumn{2}{c}{$S^D$}    \\
\cline{2-5}
  & \multicolumn{1}{c}{$P=0$}   &\multicolumn{1}{c!{\vrule width0.5pt}}{$P=1$}   &\multicolumn{1}{c}{$P=0$}    &\multicolumn{1}{c}{$P=1$}    \\ \hline
\Xhline{1.2pt}
\hline
\hline
\Xhline{1.2pt}
NonSW           &  4,512(62\%)  &  \multicolumn{1}{c!{\vrule width0.5pt}}{0(0\%)}  & \multicolumn{1}{c}{ 865(12\%)}   & \multicolumn{1}{c}{0(0\%)} \\
TrueMark       &  1,877(26\%)  & 5,012(69\%) & 5,811(80\%)   & 6,362(87\%)  \\ \cline{2-5}
TotalNum        &  \multicolumn{2}{c!{\vrule width0.5pt}}{7,285}  &\multicolumn{2}{c}{7,285}\\
\Xhline{1.2pt}
NonSW           &  9,941(52\%)& \multicolumn{1}{c!{\vrule width0.5pt}}{0(0\%)}  & 4,722(25\%)   & \multicolumn{1}{c}{0(0\%)}\\
TrueMark       &  5773(30\%)& 12,712(67\%)  & 10,603(56\%)  &15,894(84\%)  \\ \cline{2-5}
TotalNum        &  \multicolumn{2}{c!{\vrule width0.5pt}}{18,846}  &\multicolumn{2}{c}{18,846}  \\
\Xhline{1.2pt}
\end{tabular}
\end{table}


\begin{table}
\footnotesize
\caption{Examples of supervised Dirichlet priors of \emph{Reuters} documents (with seed word set $S^L$) computed by LapSWTM of Eq.\ref{Eq1} (i.e., $\alpha$) and WSPTM of Eq.\ref{Eq6} (i.e., $\alpha'$). The same parameters of Eqs.\ref{Eq1} and \ref{Eq6} used here are fixed as $\eta=10$ and $\alpha_0=0.01$, and the specific parameters of $\alpha'$ are fixed as $P=1$ (i.e., the number of pseudo-nearest neighboring categories in Eq.\ref{Eq4}) and $\tau=0.1$ (i.e., the tuning parameter in Eq.\ref{Eq4}).}   
    \centering
    \begin{tabular}{p{100pt}<{\centering}| p{40pt}<{\centering}| p{200pt}<{\centering}}
        \Xhline{1.5pt}


        % \specialrule{0em}{1pt}{1pt}
        Seed word set   & \multicolumn{2}{c}{Label (Seed word)} \\
        \Xhline{1pt}
        %% \multirow{3}{*}{$S^L$} & \multicolumn{3}{c}{\multirow{3}{210pt}{ \:\: 0 (acquisition)\:\: 1 (coffee)\:\: 2 (crude)\:\: 3 (earnings)\:\: 4 (gold) \quad\quad 5 (interest)\:\: 6 (foreign,\, exchange)\:\: 7 (ship)\:\: 8 (sugar)\:\: 9 (trade)}} \\
        \multirow{3}{*}{$S^L$ of \emph{Reuters}} & \multicolumn{2}{c}{\multirow{3}{210pt}{ \:\: 1 (acquisition)\:\: 2 (coffee)\:\: 3 (crude)\:\: 4 (earnings)\:\: 5 (gold) \quad\quad 6 (interest)\:\: 7 (foreign,\, exchange)\:\: 8 (ship)\:\: 9 (sugar)\:\: 10 (trade)}} \\
        & \multicolumn{2}{p{248pt}<{\centering}}{} \\
        & \multicolumn{2}{p{248pt}<{\centering}}{} \\
        \Xhline{1pt}
        (Label) Document  & Prior   & Prior value \\
        \Xhline{1pt}
        \multirow{9}{100pt}{\textcolor{blue}{(Label: 1)} \quad terminal sale mln did dlrs company gulf applied technologies sells units subsidiaries engaged pipeline operations 12 subject post closing adjustments}  
        % \multirow{9}{100pt}{\textcolor{blue}{(Label: 1)} \quad owned shares stock terms corp approves merger shareholders approved wholly subsidiary electric shareholder receive share}  
        & \multirow{3}{*}{$\alpha$} & \multirow{3}{*}{$[\,\textcolor{blue}{0.01},0.01,0.01,0.01,0.01,0.01,0.01,0.01,0.01,0.01\,]$}\\
        &  &  \\
        &  &  \\
        & \multirow{3}{*}{$\alpha'$ ($\rho$ = 0)} & \multirow{3}{*}{$[\,\textcolor{blue}{10.01},0.01,0.01,0.01,0.01,0.01,0.01,0.01,0.01,0.01\,]$} \\
        &  &  \\
        &  &  \\
        & \multirow{3}{*}{$\alpha'$ ($\rho$ = 0.9)} & \multirow{3}{*}{$[\,\textcolor{blue}{3.54},0.15,0.41,4.60,0.12,0.25,0.31,0.19,0.15,0.38\,]$} \\
        &  &  \\
        &  &  \\
        % \multirow{6}{100pt}{\textcolor{blue}{(Label: 1)} \quad owned shares stock terms corp approves merger shareholders approved wholly subsidiary electric shareholder receive share}  
        % & \multirow{2}{*}{$\alpha$} & \multirow{2}{*}{$[\,\textcolor{blue}{0.01},0.01,0.01,0.01,0.01,0.01,0.01,0.01,0.01,0.01\,]$}\\
        % &  &  \\
        % & \multirow{2}{*}{$\alpha'$ ($\rho$ = 0)} & \multirow{2}{*}{$[\,\textcolor{blue}{10.01},0.01,0.01,0.01,0.01,0.01,0.01,0.01,0.01,0.01\,]$} \\
        % &  &  \\
        % & \multirow{2}{*}{$\alpha'$ ($\rho$ = 0.9)} & \multirow{2}{*}{$[\,\textcolor{blue}{3.54},0.15,0.41,4.60,0.12,0.25,0.31,0.19,0.15,0.38\,]$} \\
        % &  &  \\
        \hline
        \multirow{9}{100pt}{\textcolor{blue}{(Label: 1)} \quad systems 000 shares common bought maker 677 272 following 969 643 holders 74 boards revenues pretax 232 204 pct outstanding circuit profits 1986 stock buys industries mln \textcolor{red}{exchange} dlrs 1985 board}  
        & \multirow{3}{*}{$\alpha$} & \multirow{3}{*}{$[\,\textcolor{blue}{0.01},0.01,0.01,0.01,0.01,0.01,\textcolor{red}{10.01},0.01,0.01,0.01\,]$} \\
        &  &  \\
        &  &  \\
        & \multirow{3}{*}{$\alpha'$ ($\rho$ = 0)} & \multirow{3}{*}{$[\,\textcolor{blue}{1.01},0.01,0.01,0.01,0.01,0.01,\textcolor{red}{9.01},0.01,0.01,0.01\,]$} \\
        &  &  \\
        &  &  \\
        & \multirow{3}{*}{$\alpha'$ ($\rho$ = 0.9)} & \multirow{3}{*}{$[\,\textcolor{blue}{2.64},0.15,0.41,0.460,0.12,0.25,\textcolor{red}{0.121},0.19,0.15,0.38\,]$} \\
        &  &  \\
        &  &  \\


        \Xhline{1.5pt}
    \end{tabular}
    \label{ExampleOfPrior}
\end{table}


\begin{table}[t]
\centering
\small
\caption{Statistics of datasets and seed word sets. \emph{D}: number of documents; \emph{V}: number of unique words; \emph{K}: number of categories; $S^L$ and $S^D$: average number of seed words in $S^L$ and $S^D$, respectively.}
\label{dataset}
\renewcommand\arraystretch{2.0}
\begin{tabular}{c||p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}p{0.75cm}<{\centering}}
\Xhline{1.5pt}
Dataset     &\emph{D}  &\emph{V}  &\emph{K} & $S^L$ & $S^D$ \\
\Xhline{1.2pt}
\hline
\hline
\Xhline{1.2pt}
\emph{Reuters}          &7,285	  &7,418	     & 10	  & 1.1    &6   \\ \hline
\emph{Newsgroup}         &18,846   &52,761    &20    & 1.5  &4.75 \\
\Xhline{1.5pt}
\end{tabular}
\end{table}


\begin{table*}[t]
\renewcommand\arraystretch{2.0}
\caption{Experimental results of Micro-F1. The notation ``$\ddag$'' means that the gain of WSPTM+$S^D$ is statistically significant at 0.01 level (paired sample t-test).}
\label{TableOfMicroF1}
\centering
\small
\begin{tabular}{p{37pt}!{\vrule width0.5pt}|p{18pt}<{\centering}|p{18pt}<{\centering}!{\vrule width0.5pt}p{20pt}<{\centering}|p{20pt}<{\centering}!{\vrule width0.5pt}p{20pt}<{\centering}|p{20pt}<{\centering}!{\vrule width0.5pt}p{20pt}<{\centering}|p{20pt}<{\centering}!{\vrule width0.5pt}p{21pt}<{\centering}!{\vrule width0.5pt}p{31pt}<{\centering}}
\Xhline{1.2pt}
\multirow{2}{2cm}{Dataset} &  \multicolumn{2}{c|}{\textbf{WSPTM}}  &   \multicolumn{2}{c|}{\textbf{PL-DNB}}   &   \multicolumn{2}{c|}{\textbf{STM}}  &  \multicolumn{2}{c|}{\textbf{LapSWTM}}  &  \multirow{2}{2cm}{\textbf{SVMs}} &  \multirow{2}{2cm}{\textbf{MedLDA}} \\ \cline{2-9}
& $S^L$ & $S^D$ & $S^L$ & $S^D$ & $S^L$ & $S^D$ &  $S^L$ & $S^D$ & &\\
\Xhline{1.2pt}
\hline
\hline
\Xhline{1.2pt}
\emph{Reuters}      &0.938   &\textbf{0.952}   &0.849$^\ddag$   &0.891$^\ddag$  &0.859$^\ddag$   &0.901$^\ddag$ & 0.891$^\ddag$   &0.931$^\ddag$  &0.973   &0.934 \\ \hline
\emph{Newsgroup}    &0.805   &\textbf{0.822}   &0.715$^\ddag$   &0.765$^\ddag$ &0.699$^\ddag$   &0.771$^\ddag$ &0.748$^\ddag$    &0.810$^\ddag$  &0.823   &0.811 \\
\Xhline{1.2pt}
\end{tabular}
\end{table*}

\begin{table*}[t]
\renewcommand\arraystretch{2.0}
\caption{Experimental results of Macro-F1. The notation ``$\ddag$'' means that the gain of WSPTM+$S^D$ is statistically significant at 0.01 level (paired sample t-test).}
\label{TableOfMacroF1}
\centering
\small
\begin{tabular}{p{37pt}!{\vrule width0.5pt}|p{18pt}<{\centering}|p{18pt}<{\centering}!{\vrule width0.5pt}p{20pt}<{\centering}|p{20pt}<{\centering}!{\vrule width0.5pt}p{20pt}<{\centering}|p{20pt}<{\centering}!{\vrule width0.5pt}p{20pt}<{\centering}|p{20pt}<{\centering}!{\vrule width0.5pt}p{21pt}<{\centering}!{\vrule width0.5pt}p{31pt}<{\centering}}
\Xhline{1.2pt}
\multirow{2}{2cm}{Dataset} &  \multicolumn{2}{c|}{\textbf{WSPTM}}  &   \multicolumn{2}{c|}{\textbf{PL-DNB}}   &   \multicolumn{2}{c|}{\textbf{STM}}  &  \multicolumn{2}{c|}{\textbf{LapSWTM}}  &  \multirow{2}{2cm}{\textbf{SVMs}} &  \multirow{2}{2cm}{\textbf{MedLDA}} \\ \cline{2-9}
& $S^L$ & $S^D$ & $S^L$ & $S^D$ & $S^L$ & $S^D$ &  $S^L$ & $S^D$ & &\\
\Xhline{1.2pt}
\hline
\hline
\Xhline{1.2pt}
\emph{Reuters}      &0.830   &\textbf{0.900}   &0.758$^\ddag$   &0.837$^\ddag$   &0.753$^\ddag$   &0.835$^\ddag$  &0.799$^\ddag$    &0.877$^\ddag$ &0.939   &0.916 \\ \hline
\emph{Newsgroup}    &0.759   &\textbf{0.798}   &0.677$^\ddag$   &0.731$^\ddag$    &0.669$^\ddag$   &0.737$^\ddag$ &0.693$^\ddag$    &0.783$^\ddag$  &0.816   &0.802 \\
\Xhline{1.2pt}
\end{tabular}
\end{table*}


\begin{table}[t]
\centering
\caption{Summary of the Friedman statistics $F_F$ (l=4, n=40) and the critical value of each evaluation metric.}
\renewcommand\arraystretch{1.2}
\begin{tabular}{p{80pt} p{40pt}<{\centering} p{120pt}<{\centering}}
\Xhline{1.5pt}

Evaluation metric & \emph{$F_F$}  & Critical Value($\alpha$ = 0.05) \\
\Xhline{0.5pt}

Micro-F1  & 240.0698     & \multicolumn{1}{c}{\multirow{2}{*}{2.6821}} \\
Macro-F1  & 375.8936   \\

\Xhline{1.5pt}

\end{tabular}
\label{Table_Friedman}
\end{table}



